Optimization and Abstraction: A Synergistic Approach for Analyzing Neural Network Robustness

In recent years, the notion of local robustness (or robustness for short) has emerged as a desirable property of deep neural networks. Intuitively, robustness means that small perturbations to an input do not cause the network to perform misclassifications. In this paper, we present a novel algorithm for verifying robustness properties of neural networks. Our method synergistically combines gradient-based optimization methods for counterexample search with abstraction-based proof search to obtain a sound and ({\delta}-)complete decision procedure. Our method also employs a data-driven approach to learn a verification policy that guides abstract interpretation during proof search. We have implemented the proposed approach in a tool called Charon and experimentally evaluated it on hundreds of benchmarks. Our experiments show that the proposed approach significantly outperforms three state-of-the-art tools, namely AI^2 , Reluplex, and Reluval.

==> discussion.tex <==
\section{Discussion}
\label{sec:disc}

\subsection{Limitations}
Our learned policy has two main limitations. First, since it is very expensive to train Bayesian optimization to learn a large number of parameters, we must manually identify a small set of features that best indicate how to refine and verify the input space. Second, our selection function assumes a linear combination of the learned parameters and features. However, in the optimal policy, the mapping of features to \todo{policy decisions} could be nonlinear. Both of these limitations could be addressed by a policy learned through Deep Reinforcement Learning (Deep RL). A neural network will automatically identify the most important features and learn a nonlinear mapping of those features to actions. Deep RL is a semi-supervised technique which requires a large, curated training set which may also require large manual effort. We leave this approach as interesting future work.  

